The thermodynamics of CaSiO3 in Earth's lower mantle

The lower mantle of Earth, characterized by pressures of 24-127 GPa and temperatures of 1900-2600 K, is still inaccessible to direct observations. In this work, we investigate by first principles the stability, phase diagram, elastic properties, and thermal conductivity of CaSiO3, that constitutes a significant component of Earth's lower mantle. Notably, our simulations capture in full the anharmonic ionic fluctuations arising from the extreme temperatures and pressures of the lower mantle, thanks to the use of stochastic self-consistant harmonic approximation (SSCHA). We show that the cubic phase of CaSiO3 is the stable state at the lower mantle's thermodynamic conditions. The phase boundary between the cubic and tetragonal phases is of first-order and increases linearly from 300 K to 1000 K between 12 GPa and 100 GPa. Accounting for temperature-renormalized phonon dispersions, we evaluate the speed of sound as a function of depth. Our results downplay the role of octahedral rotations on the transverse sound velocity of cubic CaSiO3, advocated in the past to explain discrepancies between theory and experiments. The lattice thermal conductivity, assessed thanks to the recently introduced Wigner formalism, shows a predominance of particle-like transport, thus justifying the use of the standard Boltzmann transport equation even in a system with such strong ionic anharmonicity.

==> bib_temporary.tex <==
@article{gupta2014characterization,
  title={\href{https://aip.scitation.org/doi/10.1063/1.4892976}{Characterization of few-layer 1T-MoSe2 and its superior performance in the visible-light induced hydrogen evolution reaction}},
  author={Gupta, Uttam and Naidu, BS and Maitra, Urmimala and Singh, Anjali and Shirodkar, Sharmila N and Waghmare, Umesh V and Rao, CNR},
  journal={APL Materials},
  volume={2},
  number={9},
  pages={092802},
  year={2014},
  publisher={American Institute of Physics}
}

